Simpler is better: A comparative study of randomized algorithms for computing the CUR decomposition

The CUR decomposition is a technique for low-rank approximation that selects small subsets of the columns and rows of a given matrix to use as bases for its column and rowspaces. It has recently attracted much interest, as it has several advantages over traditional low rank decompositions based on orthonormal bases. These include the preservation of properties such as sparsity or non-negativity, the ability to interpret data, and reduced storage requirements. The problem of finding the skeleton sets that minimize the norm of the residual error is known to be NP-hard, but classical pivoting schemes such as column pivoted QR work tend to work well in practice. When combined with randomized dimension reduction techniques, classical pivoting based methods become particularly effective, and have proven capable of very rapidly computing approximate CUR decompositions of large, potentially sparse, matrices. Another class of popular algorithms for computing CUR de-compositions are based on drawing the columns and rows randomly from the full index sets, using specialized probability distributions based on leverage scores. Such sampling based techniques are particularly appealing for very large scale problems, and are well supported by theoretical performance guarantees. This manuscript provides a comparative study of the various randomized algorithms for computing CUR decompositions that have recently been proposed. Additionally, it proposes some modifications and simplifications to the existing algorithms that leads to faster execution times.

==> format.tex <==
\RequirePackage{latexsym}
\RequirePackage{amsmath}
\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{bm}

%%%%%%%%%%%%%%% hyperref %%%%%%%%%%%%%%%
\usepackage{hyperref} %for hyperreference
\hypersetup{
    pdftoolbar=true,        % show Acrobat’s toolbar?
    pdfmenubar=true,        % show Acrobat’s menu?
    pdffitwindow=false,     % window fit to page when opened
    pdfstartview={FitH},    % fits the width of the page to the window
    pdftitle={title},    % title
    pdfauthor={Yijun Dong},     % author
    pdfsubject={Subject},   % subject of the document
    pdfcreator={Yijun Dong},   % creator of the document
    pdfproducer={Yijun Dong}, % producer of the document
    % pdfkeywords={}, % list of keywords
    pdfnewwindow=true,      % links in new window
    colorlinks=true,       % false: boxed links; true: colored links
    linkcolor=blue,          % color of internal links (change box color with linkbordercolor)
    citecolor=blue,        % color of links to bibliography
    filecolor=black,      % color of file links
    urlcolor=blue           % color of external links
}



%%%%%%%%%%%%%%% theorems %%%%%%%%%%%%%%%
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{claim}{Claim}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
    \theoremstyle{definition}
\newtheorem{definition}{Definition}
    \theoremstyle{definition}
\newtheorem{assumption}{Assumption}
    \theoremstyle{remark}
\newtheorem{remark}{Remark}
    \theoremstyle{remark}
\newtheorem{conjecture}{Conjecture}
    \theoremstyle{definition}
\newtheorem{example}{Example}
%\numberwithin{equation}{section}
%\numberwithin{figure}{section}


%%%%%%%%%%%%%%% Special characters %%%%%%%%%%%%%%%
\newcommand{\A}{\mathbb{A}}
\newcommand{\B}{\mathbb{B}}
\newcommand{\C}{\mathbb{C}} % complex field
\newcommand{\D}{\mathbb{D}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\N}{\mathbb{N}} % nature numbers
\newcommand{\Q}{\mathbb{Q}} % rational field 
\newcommand{\R}{\mathbb{R}} % real field
\newcommand{\T}{\mathbb{T}}
\newcommand{\U}{\mathbb{U}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\W}{\mathbb{W}}
\newcommand{\X}{\mathbb{X}}
\newcommand{\Y}{\mathbb{Y}}
\newcommand{\Z}{\mathbb{Z}} % integer field


% bold
\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}


\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}



\newcommand{\fA}{\mathfrak{A}}
\newcommand{\fB}{\mathfrak{B}}
\newcommand{\fC}{\mathfrak{C}}
\newcommand{\fD}{\mathfrak{D}}
\newcommand{\fE}{\mathfrak{E}}
\newcommand{\fF}{\mathfrak{F}}
\newcommand{\fG}{\mathfrak{G}}
\newcommand{\fH}{\mathfrak{H}}
\newcommand{\fI}{\mathfrak{I}}
\newcommand{\fJ}{\mathfrak{J}}
\newcommand{\fK}{\mathfrak{K}}
\newcommand{\fL}{\mathfrak{L}}
\newcommand{\fM}{\mathfrak{M}}
\newcommand{\fN}{\mathfrak{N}}
\newcommand{\fO}{\mathfrak{O}}
\newcommand{\fP}{\mathfrak{P}}
\newcommand{\fQ}{\mathfrak{Q}}
\newcommand{\fR}{\mathfrak{R}}
\newcommand{\fS}{\mathfrak{S}}
\newcommand{\fT}{\mathfrak{T}}
\newcommand{\fU}{\mathfrak{U}}
\newcommand{\fV}{\mathfrak{V}}
\newcommand{\fW}{\mathfrak{W}}
\newcommand{\fX}{\mathfrak{X}}
\newcommand{\fY}{\mathfrak{Y}}
\newcommand{\fZ}{\mathfrak{Z}}


% Greek
\newcommand{\eps}{\epsilon}
\newcommand{\veps}{\varepsilon}

\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\deltab}{\boldsymbol{\delta}}
\newcommand{\epsb}{\boldsymbol{\eps}}
\newcommand{\vepsb}{\boldsymbol{\veps}}
\newcommand{\zetab}{\boldsymbol{\zeta}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\vthetab}{\boldsymbol{\vartheta}}
\newcommand{\iotab}{\boldsymbol{\iota}}
\newcommand{\kappab}{\boldsymbol{\kappa}}
\newcommand{\vkappab}{\boldsymbol{\varkappa}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\nub}{\boldsymbol{\nu}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\omicronb}{\boldsymbol{\omicron}}
\newcommand{\pib}{\boldsymbol{\pi}}
\newcommand{\vpib}{\boldsymbol{\varpi}}
\newcommand{\rhob}{\boldsymbol{\rho}}
\newcommand{\vrhob}{\boldsymbol{\varrho}}
\newcommand{\sigmab}{\boldsymbol{\sigma}}
\newcommand{\vsigmab}{\boldsymbol{\varsigma}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\upsilonb}{\boldsymbol{\upsilon}}
\newcommand{\phib}{\boldsymbol{\phi}}
\newcommand{\vphib}{\boldsymbol{\varphi}}
\newcommand{\chib}{\boldsymbol{\chi}}
\newcommand{\psib}{\boldsymbol{\psi}}
\newcommand{\omegab}{\boldsymbol{\omega}}

\newcommand{\Alphab}{\boldsymbol{\Alpha}}
\newcommand{\Betab}{\boldsymbol{\Beta}}
\newcommand{\Gammab}{\boldsymbol{\Gamma}}
\newcommand{\Deltab}{\boldsymbol{\Delta}}
\newcommand{\Epsb}{\boldsymbol{\Epsilon}}
\newcommand{\Zetab}{\boldsymbol{\Zeta}}
\newcommand{\Etab}{\boldsymbol{\Eta}}
\newcommand{\Thetab}{\boldsymbol{\Theta}}
\newcommand{\Iotab}{\boldsymbol{\Iota}}
\newcommand{\Kappab}{\boldsymbol{\Kappa}}
\newcommand{\Lambdab}{\boldsymbol{\Lambda}}
\newcommand{\Mub}{\boldsymbol{\Mu}}
\newcommand{\Nub}{\boldsymbol{\Nu}}
\newcommand{\Xib}{\boldsymbol{\Xi}}
\newcommand{\Omicronb}{\boldsymbol{\Omicron}}
\newcommand{\Pib}{\boldsymbol{\Pi}}
\newcommand{\Rhob}{\boldsymbol{\Rho}}
\newcommand{\Sigmab}{\boldsymbol{\Sigma}}
\newcommand{\Taub}{\boldsymbol{\Tau}}
\newcommand{\Upsilonb}{\boldsymbol{\Upsilon}}
\newcommand{\Phib}{\boldsymbol{\Phi}}
\newcommand{\Chib}{\boldsymbol{\Chi}}
\newcommand{\Psib}{\boldsymbol{\Psi}}
\newcommand{\Omegab}{\boldsymbol{\Omega}}








%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%
\newcommand{\pinv}{\dagger}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}
\newcommand*{\poly}{\mathop{\mathrm{poly}}}
\newcommand*{\mean}{\mathop{\mathrm{mean}}}
\newcommand*{\median}{\mathop{\mathrm{median}}}
\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\nnz}{\mathop{\mathrm{nnz}}}
\newcommand{\prox}{\mathop{\mathrm{prox}}}
\newcommand{\proj}{\mathop{\mathrm{proj}}}
\newcommand{\ortho}{\mathop{\mathrm{ortho}}}
\newcommand{\eproof}{$\null\hfill\blacksquare$}
\newcommand{\nucnorm}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}
\newcommand{\pto}{\mathrel{\ooalign{\hfil$\mapstochar\mkern5mu$\hfil\cr$\to$\cr}}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}

\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{\partial #1^2}}
\newcommand{\pnwrt}[2]{\frac{\partial^#1}{\partial #2^#1}}
\newcommand{\pfrac}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\ppfrac}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\pnfrac}[3]{\frac{\partial^#1 #2}{\partial #3^#1}}
% proof
\renewcommand\qedsymbol{$\blacksquare$}



%%%%%%%%%%%%%%% Super/sup-scripts %%%%%%%%%%%%%%%
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\ol}[1]{\overline{#1}} % overline
\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}




%%%%%%%%%%%%%%% Short Forms %%%%%%%%%%%%%%%
\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\iid}{\emph{i.i.d.}}
\newcommand{\cf}{\emph{cf.}\ }
\newcommand{\wrt}{\emph{w.r.t.}\ }
\newcommand{\st}{\emph{s.t.}\ }


%%%%%%%%%%%%%%% Brackets %%%%%%%%%%%%%%
\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abbr}[1]{\left|#1\right|}
\newcommand{\abr}[1]{\langle#1\rangle}

\newcommand{\rsep}[2]{\left(#1 \middle| #2 \right)}
\newcommand{\ssep}[2]{\left[#1 \middle| #2 \right]}
\newcommand{\csep}[2]{\left\{#1 \middle| #2 \right\}}
\newcommand{\asep}[2]{\langle#1 \mid #2 \rangle}
\newcommand{\rsepp}[2]{\left(#1 ~\middle|~ #2 \right)}
\newcommand{\ssepp}[2]{\left[#1 ~\middle|~ #2 \right]}
\newcommand{\csepp}[2]{\left\{#1 ~\middle|~ #2 \right\}}
\newcommand{\asepp}[2]{\langle#1 ~\mid~ #2 \rangle}

\newcommand{\apar}[1]{\langle #1 \rangle}
\newcommand{\cpar}[1]{\{#1\}}
\newcommand{\bpar}[1]{\Big( #1 \Big)}
\newcommand{\Bpar}[1]{\Bigg( #1 \Bigg)}
\newcommand{\bspar}[1]{\Big[ #1 \Big]}
\newcommand{\Bspar}[1]{\Bigg[ #1 \Bigg]}
\newcommand{\bcpar}[1]{\Big\{ #1 \Big\}}
\newcommand{\Bcpar}[1]{\Bigg\{ #1 \Bigg\}}

\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\inpr}[2]{\langle #1, #2 \rangle}
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\sembrack}[1]{[\![#1]\!]}

\newcommand{\bmat}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\mat}[1]{\begin{pmatrix} #1 \end{pmatrix}}




%%%%%%%%%%%%%%% Miscellaneous %%%%%%%%%%%%%%%
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\gray}[1]{\textcolor{gray}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\bs}[1]{\boldsymbol{#1}}
\renewcommand{\b}{\textbf}
\renewcommand{\t}[1]{\text{#1}}




% Local
\newcommand{\yijun}[1]{\red{[#1]}}
\newcommand{\needref}{\textcolor{red}{\textbf{@@ref}}}
\newcommand{\cid}[2]{\wh{#1}_{*,#2}}
\newcommand{\rid}[2]{\wh{#1}_{#2,*}}
\newcommand{\cur}[2]{\wt{#1}_{#2}}
\newcommand{\tsid}[2]{\wh{#1}_{#2}}
\newcommand{\oc}[1]{{#1^{\perp}}}
\newcommand{\pobx}{\Pb_{X}}
\newcommand{\pobc}{\Pb_{C}}
\usepackage{xspace}
\newcommand{\pqr}{CPQR\xspace}
\newcommand{\plu}{LUPP\xspace}









